Exploring Collaboration Mechanisms for LLM Agents: A Social Psychology View

As Natural Language Processing (NLP) systems are increasingly employed in intricate social environments, a pressing query emerges: Can these NLP systems mirror human-esque collaborative intelligence, in a multi-agent society consisting of multiple large language models (LLMs)? This paper probes the collaboration mechanisms among contemporary NLP systems by melding practical experiments with theoretical insights. We fabricate four unique `societies' comprised of LLM agents, where each agent is characterized by a specific `trait' (easy-going or overconfident) and engages in collaboration with a distinct `thinking pattern' (debate or reflection). Through evaluating these multi-agent societies on three benchmark datasets, we discern that certain collaborative strategies not only outshine previous top-tier approaches, but also optimize efficiency (using fewer API tokens). Moreover, our results further illustrate that LLM agents manifest human-like social behaviors, such as conformity and consensus reaching, mirroring foundational social psychology theories. In conclusion, we integrate insights from social psychology to contextualize the collaboration of LLM agents, inspiring further investigations into the collaboration mechanism for LLMs. We commit to sharing our code and datasets\footnote{\url{https://github.com/zjunlp/MachineSoM}.}, hoping to catalyze further research in this promising avenue.

==> society-of-mind.tex <==
\iffalse
\bibliography{reference}
\bibliographystyle{acl_natbib}
\fi
% !TEX root = ./acl_latex.tex

% \section{Society of Mind and LLMs}
% \label{sec:SoM}
% \paragraph{What is Society of Mind?}
% Society of Mind (SoM) is a theory proposed by a computer and cognitive scientist, Marvin Minsky \cite{minsky1988society}, which seeks to explain human intelligence and cognition.
% According to this theory, the human mind and intelligence comprise numerous simple components, i.e., \textbf{\textit{agents}}.
% The individual agent is responsible for a specific aspect of mental activity, such as pattern recognition, information processing, reasoning, etc.
% Agents with different backgrounds compose into a \textbf{\textit{society}} when they interact and communicate with each other.
% The society of agents can execute tasks that are far more complicated than those achievable by any individual agent, ultimately leading to the wide range of capabilities associated with minds \cite{singh2003examining}.
% Therefore, SoM induces our thinking that multiple agents can perform excellently on different and complex tasks through collaboration processes like debate between each other and reflection with diverse interactive strategies.

% \paragraph{Why do LLMs need Society of Mind?}
% Firstly, LLM-based agents can accomplish multiple different tasks through character-playing in society.
% CAMEL \cite{DBLP:journals/corr/abs-2303-17760}, a communicative agent framework for mind exploration, assigns multiple LLMs with different roles, such as a python programmer AI assistant and a stock trader AI user, to solve specific tasks in AI society.
% Secondly, social intelligence through collaboration between LLMs can result in performance gains \cite{DBLP:journals/corr/abs-2304-12998}. Multiagents achieve better performance on reasoning and factual information extraction tasks, such as arithmetic, grade school math, chess move validity, and the like \citet{DBLP:journals/corr/abs-2305-14325}.
% In this work, we will investigate how different LLM collaboration processes, characters, and interaction strategies influence the performance in machine society with multiple LLM agents.

==> tables/llama/table_sig_main_llama.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table*}[!t] % !t, !htbp
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
Dataset & \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{Math} & \multicolumn{3}{c}{Chess Move Validity} 
\\ 

\cmidrule{2-10} 

Factor & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} 
\\ 

\midrule

Society & 3 & 0.402 & 0.752 & 3 & 1.028 & 0.382 & 3 & 2.619 & 0.188 
\\
\colorbox{gray}{Collaborative Strategy} & 7 & 2.696 & \colorbox{gray}{0.012} & 7 & 2.991 & \colorbox{gray}{0.006} & 7 & 9.784 & \colorbox{gray}{0.000} 
\\
Society\&Strategy & 21 & 1.499 & 0.089 & 21 & 0.753 & 0.770 & 21 & 0.712 & 0.814 \\ 
\bottomrule
\end{tabular}
% }
\caption{Two-way ANOVA analysis of the results of Table~\ref{table:llama_main}, \emph{using LlaMA2-chat-13B}.}
\label{table:sig_llama_main}
\end{table*}

% C(Factor1)               5.65    3.0  0.402046  0.751767
% C(Factor2)              88.40    7.0  2.695892  0.012238
% C(Factor1):C(Factor2)  147.45   21.0  1.498904  0.088729

%                         5.11875    3.0  1.028249  0.382466
% C(Factor2)              34.74375    7.0  2.991122  0.006103
% C(Factor1):C(Factor2)   26.23125   21.0  0.752758  0.770468

% C(Factor1)              16.425    3.0  1.619224  1.881335e-01
% C(Factor2)             231.575    7.0  9.783998  9.957212e-10
% C(Factor1):C(Factor2)   50.575   21.0  0.712261  8.142353e-01

==> tables/llama/table_two_agents_three_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & 
\multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & 
\multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & 
\multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} 
\\ 
\midrule
MMLU & 27.6±0.9 & 28.4±5.2 & \bf{30.4±5.0} & 29.2±4.8 & 29.6±3.0 & {27.2±4.2} & 30.0±5.3 & {30.0±4.2} 
\\
Chess Move Validity & \bf{6.0±1.4} & 6.0±4.2 & {6.0±3.2} & 6.0±4.5 & 2.8±1.8 & 4.0±3.7 & {1.6±1.7} & 2.0±2.0 
\\ 
\bottomrule
\end{tabular}
}
\caption{Accuracy of two easy-going agents in three rounds of collaboration, \emph{using LlaMA2-chat-13B}.}
\label{tab:llama13_two_agents_three_turn}
\end{table*}




\begin{comment}
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & \multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & \multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & \multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} \\ \midrule
MMLU & \colorbox{Mycolor1}{\textbf{64.8±4.4}} & \colorbox{Mycolor3}{64.8±5.8} & 58.4±3.0 & 51.6±3.8 & \colorbox{Mycolor2}{38.0±3.7} & 42.0±2.4 & 54.0±5.8 & 41.2±5.2 
\\ 
MATH & \colorbox{Mycolor3}{50.8±5.4} & 45.2±7.0 & 48.8±9.4 & 44.8±3.3 & 49.2±8.7 & \colorbox{Mycolor1}{\textbf{51.2±2.3}} & 48.4±6.5 & \colorbox{Mycolor2}{40.8±6.1} 
\\
Chess Move Validity & \colorbox{Mycolor3}{48.4±3.3} & \colorbox{Mycolor1}{\textbf{49.6±4.6}} & 46.0±3.5 & 36.8±4.1 & 38.8±3.3 & 27.2±3.9 & 38.0±6.3 & \colorbox{Mycolor2}{14.0±4.7} 
\\ 
\bottomrule
\end{tabular}
}
\caption{Performance of three easy-going agents in three rounds of collaboration.}
\label{tab:three_agents_three_turn}
\end{table}
\end{comment}

==> tables/llama/table_two_agents_two_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & $p_0p_0$ & $p_0p_1$ & $p_1p_0$ & $p_1p_1$ \\ \midrule
MMLU  & \bf{30.4±3.8} & 28.0±5.1 & 28.0±3.1 & 29.0±4.0 \\
Chess Move Validity & \bf{5.6±3.5} & 5.2±3.8 & 3.2±2.9 & 0.8±1.4 \\ \bottomrule
\end{tabular}
% }
\caption{Accuracy of two easy-going agents in two rounds of collaboration, \emph{using LlaMA2-chat-13B}.}
\label{tab:llama13_two_agents_two_turn}
\end{table*}

==> tables/llama70/table_sig_main_llama70.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
Dataset & \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{Math} & \multicolumn{3}{c}{Chess Move Validity} 
\\ 

\cmidrule{2-10} 

Factor & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} 
\\ 

\midrule

Society & 3 & 0.659 & 0.578 & 3 & 2.072 & 0.107 & 3 & 0.073 & 0.974
\\
\colorbox{gray}{Collaborative Strategy} & 7 & 13.782 & \colorbox{gray}{0.000} & 7 & 2.774 & \colorbox{gray}{0.010} & 7 & 15.038 & \colorbox{gray}{0.000} 
\\
Society\&Strategy & 21 & 2.400 & \colorbox{gray}{0.001} & 21 & 0.858 & 0.644 & 21 & 1.091 & 0.366 \\ 
\bottomrule
\end{tabular}
% }
\caption{Two-way ANOVA analysis of the results in Table~\ref{table:llama70_main}, \emph{using LlaMA2-chat-70B}.}
\label{table:sig_llama70_main}
\end{table*}

% ====================llama70====================
% ====================main====================
%                               sum_sq     df          F        PR(>F)
% C(Society)                     9.125    3.0   0.659440  5.784849e-01
% C(Collaboration)             444.975    7.0  13.781649  3.277748e-13
% C(Society):C(Collaboration)  232.475   21.0   2.400052  1.479648e-03
% Residual                     590.400  128.0        NaN           NaN
% ====================llama70====================
% ====================main====================
%                                 sum_sq     df         F    PR(>F)
% C(Society)                     7.16875    3.0  2.072267  0.107121
% C(Collaboration)              22.39375    7.0  2.774293  0.010182
% C(Society):C(Collaboration)   20.78125   21.0  0.858175  0.643875
% Residual                     147.60000  128.0       NaN       NaN
% ====================llama70====================
% ====================main====================
%                                 sum_sq     df          F        PR(>F)
% C(Society)                     0.86875    3.0   0.072851  9.744289e-01
% C(Collaboration)             418.44375    7.0  15.038410  3.149276e-14
% C(Society):C(Collaboration)   91.08125   21.0   1.091120  3.656842e-01
% Residual                     508.80000  128.0        NaN           NaN

==> tables/llama70/table_two_agents_three_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & \multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & \multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & \multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} \\ \midrule
MMLU & 35.2±4.6 & \bf{35.6±4.3} & 28.8±3.9 & 33.2±3.6 & 22.0±6.2 & 16.8±5.4 & 23.6±3.3 & 19.6±5.2 \\
Chess Move Validity & 3.2±3.0 & \bf{5.2±1.8} & 3.2±3.4 & 0.4±0.9 & 4.8±2.3 & 5.2±3.0 & 2.8±3.4 & 1.6±1.7 \\ 
\bottomrule
\end{tabular}
}
\caption{Accuracy of two easy-going agents in three rounds of collaboration, \emph{using LlaMA2-chat-70B}.}
\label{tab:llama70_two_agents_three_turn}
\end{table*}

==> tables/llama70/table_two_agents_two_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & $p_0p_0$ & $p_0p_1$ & $p_1p_0$ & $p_1p_1$ \\ \midrule
MMLU  & \bf{35.4±5.7} & 31.6±2.5 & 20.2±4.9 & 19.4±2.8 \\
Chess Move Validity & 3.2±2.9 & 2.8±1.7 & \bf{5.6±3.0} & 3.2±2.5 \\ \bottomrule
\end{tabular}
% }
\caption{Accuracy of two easy-going agents in two rounds of collaboration, \emph{using LlaMA2-chat-70B}.}
\label{tab:llama70_two_agents_two_turn}
\end{table*}

==> tables/mixtral/table_sig_agents_mixtral.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table}[!htbp] % !t
\centering
\vspace{-4mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\toprule
 & \multicolumn{1}{r}{MMLU} & \multicolumn{1}{r}{Chess Move Validity} \\
Collaborative Strategy & \multicolumn{1}{r}{p-value} & \multicolumn{1}{r}{p-value} \\ \midrule
$p_0p_0p_0$ & \colorbox{gray}{0.010} & \colorbox{gray}{0.000} \\
$p_0p_0p_1$ & {0.057} & \colorbox{gray}{0.025} \\
$p_0p_1p_0$ & \colorbox{gray}{0.001} & {0.658} \\
$p_0p_1p_1$ & \colorbox{gray}{0.027} & \colorbox{gray}{0.016} \\
$p_1p_0p_0$ & {0.091} & \colorbox{gray}{0.028} \\
$p_1p_0p_1$ & \colorbox{gray}{0.001} & \colorbox{gray}{0.000} \\
$p_1p_1p_0$ & \colorbox{gray}{0.003} & \colorbox{gray}{0.001} \\
$p_1p_1p_1$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\
% \colorbox{gray}
\bottomrule
\end{tabular}
}
\caption{One-way ANOVA analysis of results in Figure~\ref{fig:mixtral:agent} (different numbers of agents), \emph{on Mixtral 8$\times$7B}.}
\label{table:sig_mixtral_agent}
\end{table}


% ====================mixtral,mmlu====================
% ====================agent====================
% 0.009568895350948738,$p_0p_0p_0$
% 0.057288048199201046,$p_0p_0p_1$
% 0.0014248697518827258,$p_0p_1p_0$
% 0.026533739027373528,$p_0p_1p_1$
% 0.09071182599263448,$p_1p_0p_0$
% 0.0012627875444055526,$p_1p_0p_1$
% 0.0029625466108906978,$p_1p_1p_0$
% 9.802432904284279e-05,$p_1p_1p_1$
% ====================mixtral,chess====================
% ====================agent====================
% 0.00048153677441659505,$p_0p_0p_0$
% 0.024564146834054834,$p_0p_0p_1$
% 0.6576233268237203,$p_0p_1p_0$
% 0.016231723395618885,$p_0p_1p_1$
% 0.027746638545663022,$p_1p_0p_0$
% 0.0003273949476836778,$p_1p_0p_1$
% 0.0013281159323466159,$p_1p_1p_0$
% 0.00047900905494712245,$p_1p_1p_1$

==> tables/mixtral/table_sig_main_mixtral.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
Dataset & \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{Math} & \multicolumn{3}{c}{Chess Move Validity} 
\\ 

\cmidrule{2-10} 

Factor & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} 
\\ 

\midrule

Society & 3 & 1.377 & 0.253 & 3 & 1.037 & 0.379 & 3 & 8.183 & \colorbox{gray}{0.000}
\\
\colorbox{gray}{Collaborative Strategy} & 7 & 1.939 & {0.069} & 7 & 2.654 & \colorbox{gray}{0.013} & 7 & 6.182 & \colorbox{gray}{0.000} 
\\
Society\&Strategy & 21 & 0.886 & {0.609} & 21 & 0.945 & 0.534 & 21 & 1.607 & 0.057 \\ 
\bottomrule
\end{tabular}
% }
\caption{Two-way ANOVA analysis of the results of Table~\ref{table:mixtral_main}, \emph{using Mixtral 8$\times$7B}.}
\label{table:sig_mixtral_main}
\end{table*}

% ====================main====================
%                              sum_sq     df         F    PR(>F)
% C(Society)                    22.15    3.0  1.376845  0.252841
% C(Collaboration)              72.80    7.0  1.939394  0.068503
% C(Society):C(Collaboration)   99.75   21.0  0.885781  0.609220
% Residual                     686.40  128.0       NaN       NaN
% ====================mixtral====================
% ====================main====================
%                                  sum_sq     df         F    PR(>F)
% C(Society)                     25.11875    3.0  1.036894  0.378641
% C(Collaboration)              150.04375    7.0  2.654467  0.013483
% C(Society):C(Collaboration)   160.33125   21.0  0.945489  0.534442
% Residual                     1033.60000  128.0       NaN       NaN
% ====================mixtral====================
% ====================main====================
%                               sum_sq     df         F    PR(>F)
% C(Society)                   104.025    3.0  8.182891  0.000050
% C(Collaboration)             183.375    7.0  6.182048  0.000003
% C(Society):C(Collaboration)  142.975   21.0  1.606686  0.057259
% Residual                     542.400  128.0       NaN       NaN

==> tables/mixtral/table_sig_turn_mixtral.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table}[!htbp] % !t
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\toprule
 & MMLU & Chess Move Validity \\
Collaborative Strategy & p-value & p-value \\ \midrule
$p_0p_0p_0p_0$ & \colorbox{gray}{0.042} & {0.911} \\
$p_0p_0p_0p_1$ & {0.974} & {0.832} \\
$p_0p_0p_1p_0$ & {0.924} & {0.708} \\
$p_0p_0p_1p_1$ & {0.640} & {0.845} \\
$p_0p_1p_0p_0$ & {0.992} & {0.792} \\
$p_0p_1p_0p_1$ & {0.721} & {0.107} \\
$p_0p_1p_1p_0$ & {0.400} & {0.992} \\
$p_0p_1p_1p_1$ & {0.977} & {0.697} \\
$p_1p_0p_0p_0$ & {0.554} & {0.881} \\
$p_1p_0p_0p_1$ & {0.724} & {0.736} \\
$p_1p_0p_1p_0$ & {0.821} & {0.932} \\
$p_1p_0p_1p_1$ & {0.906} & {0.754} \\
$p_1p_1p_0p_0$ & {0.901} & {0.052} \\
$p_1p_1p_0p_1$ & {0.612} & {0.923} \\
$p_1p_1p_1p_0$ & {0.759} & {0.382} \\
$p_1p_1p_1p_1$ & {0.903} & {0.978} \\
\bottomrule
% \colorbox{gray}
\end{tabular}
}
\caption{
One-way ANOVA analysis of the results in Figure~\ref{fig:mixtral:round_10_on_mmlu},~\ref{fig:mixtral:round_10_on_math},~\ref{fig:mixtral:round_10_on_chess} (different rounds), \emph{using Mixtral 8$\times$7B}. % \ref{fig:mixtral:turn}
}
\label{table:sig_mixtral_turn}
\end{table}

% ====================mixtral,mmlu====================
% ====================turn====================
% 0.04207066471868619,$p_0p_0p_0p_0$
% 0.9735697979717955,$p_0p_0p_0p_1$
% 0.9236044711599674,$p_0p_0p_1p_0$
% 0.6401186856511157,$p_0p_0p_1p_1$
% 0.9916025674229988,$p_0p_1p_0p_0$
% 0.7209415058949871,$p_0p_1p_0p_1$
% 0.39982223011458584,$p_0p_1p_1p_0$
% 0.9765176956769891,$p_0p_1p_1p_1$
% 0.5539723867550492,$p_1p_0p_0p_0$
% 0.7243109717446727,$p_1p_0p_0p_1$
% 0.8214050438400375,$p_1p_0p_1p_0$
% 0.9062154679702037,$p_1p_0p_1p_1$
% 0.9014515489931202,$p_1p_1p_0p_0$
% 0.6118701414831765,$p_1p_1p_0p_1$
% 0.7585362874581871,$p_1p_1p_1p_0$
% 0.9025180399092141,$p_1p_1p_1p_1$
% ====================mixtral,chess====================
% ====================turn====================
% 0.9107303799179635,$p_0p_0p_0p_0$
% 0.8320840540416952,$p_0p_0p_0p_1$
% 0.7075168375442192,$p_0p_0p_1p_0$
% 0.8450599420776115,$p_0p_0p_1p_1$
% 0.7916092386650722,$p_0p_1p_0p_0$
% 0.1065409910560567,$p_0p_1p_0p_1$
% 0.9922829955771227,$p_0p_1p_1p_0$
% 0.6974074624184645,$p_0p_1p_1p_1$
% 0.881085127042047,$p_1p_0p_0p_0$
% 0.7363080909190604,$p_1p_0p_0p_1$
% 0.9320376774054827,$p_1p_0p_1p_0$
% 0.7541608295953592,$p_1p_0p_1p_1$
% 0.05193973416234263,$p_1p_1p_0p_0$
% 0.923053659265602,$p_1p_1p_0p_1$
% 0.38230874012327243,$p_1p_1p_1p_0$
% 0.9775710180360103,$p_1p_1p_1p_1$

==> tables/mixtral/table_two_agents_three_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & \multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & \multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & \multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} \\ \midrule
MMLU & 53.6±2.6 & 50.8±6.1 & 54.4±1.7 & \bf{54.8±5.2} & 52.8±5.0 & 49.6±3.0 & 53.6±4.8 & 46.0±2.8 \\
Chess Move Validity & 17.2±3.6 & 18.8±1.8 & \bf{22.0±3.7} & 18.8±6.6 & 21.2±3.6 & 16.8±4.8 & 15.2±3.6 & 9.2±2.3 \\ 
\bottomrule
\end{tabular}
}
\caption{Accuracy of two easy-going agents in three rounds of collaboration, \emph{using Mixtral-8$\times$7B}.}
\label{tab:mixtral_two_agents_three_turn}
\end{table*}

==> tables/mixtral/table_two_agents_two_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & $p_0p_0$ & $p_0p_1$ & $p_1p_0$ & $p_1p_1$ \\ \midrule
MMLU  & 50.8±5.0 & \bf{54.8±4.5} & 51.0±4.6 & 48.2±5.7 \\
Chess Move Validity & 17.4±3.3 & \bf{18.6±5.5} & 18.2±3.3 & 9.6±3.2 \\ \bottomrule
\end{tabular}
% }
\caption{Accuracy of two easy-going agents in two rounds of collaboration, \emph{using Mixtral-8$\times$7B}.}
\label{tab:mixtral_two_agents_two_turn}
\end{table*}

==> tables/qwen-max/table_sig_agents_qwen.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table}[!htbp] % !t
\centering
\vspace{-4mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\toprule
 & \multicolumn{1}{r}{MMLU} & \multicolumn{1}{r}{Chess Move Validity} \\
Collaborative Strategy & \multicolumn{1}{r}{p-value} & \multicolumn{1}{r}{p-value} \\ \midrule
$p_0p_0p_0$ & {0.077} & {0.512} \\
$p_0p_0p_1$ & {0.141} & \colorbox{gray}{0.036} \\
$p_0p_1p_0$ & \colorbox{gray}{0.003} & \colorbox{gray}{0.006} \\
$p_0p_1p_1$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.015} \\
$p_1p_0p_0$ & {0.146} & \colorbox{gray}{0.000} \\
$p_1p_0p_1$ & \colorbox{gray}{0.009} & \colorbox{gray}{0.001} \\
$p_1p_1p_0$ & {0.463} & \colorbox{gray}{0.000} \\
$p_1p_1p_1$ & \colorbox{gray}{0.001} & \colorbox{gray}{0.005} \\
% \colorbox{gray}
\bottomrule
\end{tabular}
}
\caption{One-way ANOVA analysis of the results in Figure~\ref{fig:qwen:agent} (different numbers of agents), \emph{on Qwen 72B}.}
\label{table:sig_qwen_agent}
\end{table}


% ====================qwen-max-1201,mmlu====================
% ====================agent====================
% 0.07747189213780599,$p_0p_0p_0$
% 0.14142218810712381,$p_0p_0p_1$
% 0.0033363009699852,$p_0p_1p_0$
% 2.951000108707218e-05,$p_0p_1p_1$
% 0.14577703289322064,$p_1p_0p_0$
% 0.00861087280742427,$p_1p_0p_1$
% 0.46283294388439317,$p_1p_1p_0$
% 0.0012079071173635872,$p_1p_1p_1$
% ====================qwen-max-1201,chess====================
% ====================agent====================
% 0.5123575050522824,$p_0p_0p_0$
% 0.03573358350301119,$p_0p_0p_1$
% 0.006293848997529489,$p_0p_1p_0$
% 0.014949185473629749,$p_0p_1p_1$
% 8.983685174713589e-05,$p_1p_0p_0$
% 0.0012375634476505526,$p_1p_0p_1$
% 8.221791148824887e-05,$p_1p_1p_0$
% 0.005318378576451585,$p_1p_1p_1$

==> tables/qwen-max/table_sig_main_qwen.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
Dataset & \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{Math} & \multicolumn{3}{c}{Chess Move Validity} 
\\ 

\cmidrule{2-10} 

Factor & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} 
\\ 

\midrule

Society & 3 & 0.918 & 0.434 & 3 & 0.635 & 0.594 & 3 & 0.953 & {0.417}
\\
\colorbox{gray}{Collaborative Strategy} & 7 & 3.938 & \colorbox{gray}{0.001}  & 7 & 6.239 & \colorbox{gray}{0.000} & 7 & 77.755 & \colorbox{gray}{0.000} 
\\
Society\&Strategy & 21 & 1.405 & {0.128} & 21 & 1.421 & 0.120 & 21 & 0.738 & 0.787 \\ 
\bottomrule
\end{tabular}
% }
\caption{Two-way ANOVA analysis of the results of Table~\ref{table:qwen_main}, \emph{using Qwen 72B}.}
\label{table:sig_qwen_main}
\end{table*}

% ====================qwen-max-1201====================
% ====================main====================
%                               sum_sq     df         F    PR(>F)
% C(Society)                    17.025    3.0  0.918099  0.434199
% C(Collaboration)             170.375    7.0  3.937599  0.000634
% C(Society):C(Collaboration)  182.375   21.0  1.404979  0.127600
% Residual                     791.200  128.0       NaN       NaN
% ====================qwen-max-1201====================
% ====================main====================
%                                 sum_sq     df         F    PR(>F)
% C(Society)                    11.11875    3.0  0.634904  0.593838
% C(Collaboration)             254.94375    7.0  6.239064  0.000003
% C(Society):C(Collaboration)  174.23125   21.0  1.421281  0.119964
% Residual                     747.20000  128.0       NaN       NaN
% ====================qwen-max-1201====================
% ====================main====================
%                                sum_sq     df          F        PR(>F)
% C(Society)                     19.925    3.0   0.953492  4.169613e-01
% C(Collaboration)             3791.275    7.0  77.754791  4.963649e-43
% C(Society):C(Collaboration)   107.975   21.0   0.738149  7.866730e-01
% Residual                      891.600  128.0        NaN           NaN

==> tables/qwen-max/table_sig_turn_qwen.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table}[!htbp] % !t
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\toprule
 & MMLU & Chess Move Validity \\
Collaborative Strategy & p-value & p-value \\ \midrule
$p_0p_0p_0p_0$ & {0.833} & {0.957} \\
$p_0p_0p_0p_1$ & {0.351} & {0.639} \\
$p_0p_0p_1p_0$ & {0.700} & {0.730} \\
$p_0p_0p_1p_1$ & {0.901} & {0.769} \\
$p_0p_1p_0p_0$ & {0.900} & {0.741} \\
$p_0p_1p_0p_1$ & {0.573} & {0.603} \\
$p_0p_1p_1p_0$ & {0.844} & {1.000} \\
$p_0p_1p_1p_1$ & {0.560} & {0.848} \\
$p_1p_0p_0p_0$ & {0.921} & {0.358} \\
$p_1p_0p_0p_1$ & {0.300} & {0.722} \\
$p_1p_0p_1p_0$ & {0.907} & {0.407} \\
$p_1p_0p_1p_1$ & {0.843} & \colorbox{gray}{0.010} \\
$p_1p_1p_0p_0$ & {0.303} & \colorbox{gray}{0.046} \\
$p_1p_1p_0p_1$ & {0.287} & \colorbox{gray}{0.009} \\
$p_1p_1p_1p_0$ & {0.464} & \colorbox{gray}{0.003} \\
$p_1p_1p_1p_1$ & {0.939} & {0.766} \\ 
\bottomrule
% \colorbox{gray}
\end{tabular}
}
\caption{
One-way ANOVA analysis of the results in Figure~\ref{fig:qwen:round_10_on_mmlu},~\ref{fig:qwen:round_10_on_math},~\ref{fig:qwen:round_10_on_chess} (different rounds), \emph{using Qwen 72B}. % ~\ref{fig:qwen:turn}
}
\label{table:sig_qwen_turn}
\end{table}

% ====================qwen-max-1201,mmlu====================
% ====================turn====================
% 0.8328530188439995,$p_0p_0p_0p_0$
% 0.3512980316160002,$p_0p_0p_0p_1$
% 0.7002958331045976,$p_0p_0p_1p_0$
% 0.9014231685131943,$p_0p_0p_1p_1$
% 0.9002037934238675,$p_0p_1p_0p_0$
% 0.5731026687716715,$p_0p_1p_0p_1$
% 0.8444875698403315,$p_0p_1p_1p_0$
% 0.5596869000017768,$p_0p_1p_1p_1$
% 0.9214627805667257,$p_1p_0p_0p_0$
% 0.2999845898617094,$p_1p_0p_0p_1$
% 0.9066001979575335,$p_1p_0p_1p_0$
% 0.8428915740363214,$p_1p_0p_1p_1$
% 0.3031202896676407,$p_1p_1p_0p_0$
% 0.28722120128641987,$p_1p_1p_0p_1$
% 0.46411165624077017,$p_1p_1p_1p_0$
% 0.9389281378676239,$p_1p_1p_1p_1$
% ====================qwen-max-1201,chess====================
% ====================turn====================
% 0.9573451770881506,$p_0p_0p_0p_0$
% 0.6390734786037771,$p_0p_0p_0p_1$
% 0.7299156419974693,$p_0p_0p_1p_0$
% 0.7686989818129334,$p_0p_0p_1p_1$
% 0.7413087920942849,$p_0p_1p_0p_0$
% 0.6034135192892812,$p_0p_1p_0p_1$
% 1.0,$p_0p_1p_1p_0$
% 0.8484078147866152,$p_0p_1p_1p_1$
% 0.3583694333622422,$p_1p_0p_0p_0$
% 0.7221198143360507,$p_1p_0p_0p_1$
% 0.40702784958898724,$p_1p_0p_1p_0$
% 0.010319343862720128,$p_1p_0p_1p_1$
% 0.04558202527017638,$p_1p_1p_0p_0$
% 0.008863370723473518,$p_1p_1p_0p_1$
% 0.0032392574033488957,$p_1p_1p_1p_0$
% 0.7658947081406727,$p_1p_1p_1p_1$

==> tables/qwen-max/table_two_agents_three_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & \multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & \multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & \multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} \\ \midrule
MMLU & \bf{60.8±5.6} & 59.6±2.6 & 52.4±2.6 & 55.2±4.2 & 58.4±4.3 & 51.2±4.6 & 58.8±5.0 & 52.8±7.8 \\
Chess Move Validity & \bf{33.2±3.0} & 28.0±5.8 & 26.0±3.2 & 20.0±8.1 & 10.0±2.5 & 13.2±3.4 & 4.0±3.2 & 4.0±1.4 \\ 
\bottomrule
\end{tabular}
}
\caption{Accuracy of two easy-going agents in three rounds of collaboration, \emph{using Qwen 72B.}}
\label{tab:qwen_two_agents_three_turn}
\end{table*}

==> tables/qwen-max/table_two_agents_two_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & $p_0p_0$ & $p_0p_1$ & $p_1p_0$ & $p_1p_1$ \\ \midrule
MMLU  & \bf{58.6±4.7} & 53.8±4.3 & 53.4±5.0 & 54.6±6.5 \\
Chess Move Validity & \bf{30.6±4.1} & 20.8±5.8 & 9.0±3.2 & 3.4±3.0 \\ \bottomrule
\end{tabular}
% }
\caption{Accuracy of two easy-going agents in two rounds of collaboration, \emph{using Qwen 72B}.}
\label{tab:qwen_two_agents_two_turn}
\end{table*}

==> tables/table_sig_agent.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table}[!t] % !t, !htbp
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\toprule
 & \multicolumn{1}{r}{MMLU} & \multicolumn{1}{r}{Chess Move Validity} \\
Collaborative Strategy & \multicolumn{1}{r}{p-value} & \multicolumn{1}{r}{p-value} \\ \midrule
% $p_0p_0p_0$ & 0.392 & 0.475 \\
% $p_0p_0p_1$ & 0.845 & 0.078 \\
% $p_0p_1p_0$ & \colorbox{gray}{0.023} & 0.116 \\
% $p_0p_1p_1$ & 1.000 & 0.794 \\
% $p_1p_0p_0$ & 0.883 & \colorbox{gray}{0.028} \\
% $p_1p_0p_1$ & 0.321 & 0.535 \\
% $p_1p_1p_0$ & \colorbox{gray}{0.037} & 0.128 \\
% $p_1p_1p_1$ & 0.068 & 0.085 
$p_0p_0p_0$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\
$p_0p_0p_1$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\
$p_0p_1p_0$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\
$p_0p_1p_1$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\
$p_1p_0p_0$ & \colorbox{gray}{0.010} & \colorbox{gray}{0.000} \\
$p_1p_0p_1$ & \colorbox{gray}{0.021} & \colorbox{gray}{0.000} \\
$p_1p_1p_0$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\
$p_1p_1p_1$ & \colorbox{gray}{0.000} & \colorbox{gray}{0.000} \\ 
\bottomrule
\end{tabular}
}
\caption{
One-way ANOVA analysis of results in Figure~\ref{fig:agent_10_on_numbers} (different numbers of agents), using \emph{ChatGPT}. % Figure~\ref{fig:agent}
}
\label{table:sig_agent}
\end{table}

==> tables/table_sig_main.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table*}[!htbp] % !t
\centering
\small
\begin{tabular}{llllllllll}
\toprule
Dataset & \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{Math} & \multicolumn{3}{c}{Chess Move Validity} 
\\ 

\cmidrule{2-10} 

Factor & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{df} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} 
\\ 

\midrule

Society & 3 & 0.173 & 0.914 & 3 & 0.739 & 0.531 & 3 & 2.117 & 0.101 
\\
\colorbox{gray}{Collaborative Strategy} & 7 & 84.934 & \colorbox{gray}{0.000} & 7 & 3.551 & \colorbox{gray}{0.002} & 7 & 71.497 & \colorbox{gray}{0.000} 
\\
Society\&Strategy & 21 & 1.174 & 0.285 & 21 & 1.115 & 0.341 & 21 & 1.024 & 0.439 
\\ 
\bottomrule
\end{tabular}
\caption{
Two-way ANOVA analysis of the results of Table~\ref{table:main}, using \emph{ChatGPT}.
}
\label{table:sig_main}
\end{table*}

==> tables/table_sig_turn.tex <==
\definecolor{gray}{HTML}{CCCCCC}
\begin{table}[!t] % !t, !htbp
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\toprule
 & MMLU & Chess Move Validity \\
Collaborative Strategy & p-value & p-value \\ \midrule
$p_0p_0p_0p_0$ & 0.374 & 0.937 \\
$p_0p_0p_0p_1$ & 0.836 & 0.881 \\
$p_0p_0p_1p_0$ & 0.267 & 0.188 \\
$p_0p_0p_1p_1$ & 0.072 & 0.116 \\
$p_0p_1p_0p_0$ & 0.270 & 0.069 \\
$p_0p_1p_0p_1$ & 0.456 & 0.303 \\
$p_0p_1p_1p_0$ & \colorbox{gray}{0.007} & \colorbox{gray}{0.013} \\
$p_0p_1p_1p_1$ & \colorbox{gray}{0.030} & \colorbox{gray}{0.000} \\
$p_1p_0p_0p_0$ & 0.589 & 0.223 \\
$p_1p_0p_0p_1$ & 0.500 & 0.208 \\
$p_1p_0p_1p_0$ & \colorbox{gray}{0.004} & 0.082 \\
$p_1p_0p_1p_1$ & \colorbox{gray}{0.002} & \colorbox{gray}{0.047} \\
$p_1p_1p_0p_0$ & 0.471 & \colorbox{gray}{0.000} \\
$p_1p_1p_0p_1$ & 0.652 & \colorbox{gray}{0.003} \\
$p_1p_1p_1p_0$ & 0.109 & \colorbox{gray}{0.001} \\
$p_1p_1p_1p_1$ & 0.098 & 0.146 \\ \bottomrule
\end{tabular}
}
\caption{
One-way ANOVA analysis of the results in Figure~\ref{fig:round_10_on_math},~\ref{fig:round_10_on_mmlu},~\ref{fig:round_10_on_chess} (different rounds), using \emph{ChatGPT}. 
% Figure~\ref{fig:round}
}
\label{table:sig_turn}
\end{table}

==> tables/table_two_agents_three_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & 
\multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & 
\multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & 
\multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} 
\\ 
\midrule
MMLU & \bf{56.4}±1.7 & 52.8±1.8 & 44.8±7.4 & 32.4±3.6 & 26.8±5.0 & 26.0±3.7 & 38.8±4.1 & 24.8±6.9 
\\
MATH & 36.0±3.7 & \bf{37.2}±6.4 & 34.0±1.4 & 32.4±3.3 & 33.2±4.8 & 30.8±3.3 & 26.8±3.3 & 27.2±4.1 
\\
Chess Move Validity & \bf{38.0}±1.4 & 36.4±5.4 & 30.4±6.2 & 29.6±3.8 & 27.6±4.6 & 21.6±6.8 & 26.0±1.4 & 16.0±2.8 
\\ 
\bottomrule
\end{tabular}
}
\caption{Accuracy of two easy-going agents in three rounds of collaboration, using \emph{ChatGPT}.}
\label{tab:two_agents_three_turn}
\end{table*}




\begin{comment}
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{1}{c}{$p_0p_0p_0$} & \multicolumn{1}{c}{$p_0p_0p_1$} & \multicolumn{1}{c}{$p_0p_1p_0$} & \multicolumn{1}{c}{$p_0p_1p_1$} & \multicolumn{1}{c}{$p_1p_0p_0$} & \multicolumn{1}{c}{$p_1p_0p_1$} & \multicolumn{1}{c}{$p_1p_1p_0$} & \multicolumn{1}{c}{$p_1p_1p_1$} \\ \midrule
MMLU & \colorbox{Mycolor1}{\textbf{64.8±4.4}} & \colorbox{Mycolor3}{64.8±5.8} & 58.4±3.0 & 51.6±3.8 & \colorbox{Mycolor2}{38.0±3.7} & 42.0±2.4 & 54.0±5.8 & 41.2±5.2 
\\ 
MATH & \colorbox{Mycolor3}{50.8±5.4} & 45.2±7.0 & 48.8±9.4 & 44.8±3.3 & 49.2±8.7 & \colorbox{Mycolor1}{\textbf{51.2±2.3}} & 48.4±6.5 & \colorbox{Mycolor2}{40.8±6.1} 
\\
Chess Move Validity & \colorbox{Mycolor3}{48.4±3.3} & \colorbox{Mycolor1}{\textbf{49.6±4.6}} & 46.0±3.5 & 36.8±4.1 & 38.8±3.3 & 27.2±3.9 & 38.0±6.3 & \colorbox{Mycolor2}{14.0±4.7} 
\\ 
\bottomrule
\end{tabular}
}
\caption{Performance of three easy-going agents in three rounds of collaboration.}
\label{tab:three_agents_three_turn}
\end{table}
\end{comment}

==> tables/table_two_agents_two_turns.tex <==
\begin{table*}[!htbp] % !t
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & $p_0p_0$ & $p_0p_1$ & $p_1p_0$ & $p_1p_1$ \\ \midrule
MMLU  & \bf{56.7}±3.1 & 43.8±6.7 & 23.6±4.3 & 33.0±7.8 \\
MATH  & \bf{35.1}±4.0 & 32.2±4.6 & 29.2±6.1 & 24.8±5.0 \\
Chess Move Validity & \bf{36.7}±3.5 & 31.0±6.7 & 25.8±5.6 & 23.6±3.9 \\ \bottomrule
\end{tabular}
% }
\caption{Accuracy of two easy-going agents in two rounds of collaboration, using \emph{ChatGPT}.}
\label{tab:two_agents_two_turn}
\end{table*}
